Prometheus: Inducing Fine-grained Evaluation Capability in Language Models

Recently, using a powerful proprietary Large Language Model (LLM) (e.g., GPT-4) as an evaluator for long-form responses has become the de facto standard. However, for practitioners with large-scale evaluation tasks and custom criteria in consideration (e.g., child-readability), using proprietary LLMs as an evaluator is unreliable due to the closed-source nature, uncontrolled versioning, and prohibitive costs. In this work, we propose Prometheus, a fully open-source LLM that is on par with GPT-4's evaluation capabilities when the appropriate reference materials (reference answer, score rubric) are accompanied. We first construct the Feedback Collection, a new dataset that consists of 1K fine-grained score rubrics, 20K instructions, and 100K responses and language feedback generated by GPT-4. Using the Feedback Collection, we train Prometheus, a 13B evaluator LLM that can assess any given long-form text based on customized score rubric provided by the user. Experimental results show that Prometheus scores a Pearson correlation of 0.897 with human evaluators when evaluating with 45 customized score rubrics, which is on par with GPT-4 (0.882), and greatly outperforms ChatGPT (0.392). Furthermore, measuring correlation with GPT-4 with 1222 customized score rubrics across four benchmarks (MT Bench, Vicuna Bench, Feedback Bench, Flask Eval) shows similar trends, bolstering Prometheus's capability as an evaluator LLM. Lastly, Prometheus achieves the highest accuracy on two human preference benchmarks (HHH Alignment & MT Bench Human Judgment) compared to open-sourced reward models explicitly trained on human preference datasets, highlighting its potential as an universal reward model. We open-source our code, dataset, and model at https://kaistai.github.io/prometheus/.

==> figures/main/human_eval_combined.tex <==
\begin{figure*}[t!]
 \begin{subfigure}[b]{0.5\textwidth}
\centering
    \includegraphics[width=\textwidth]{figures/resources/human_eval_score_correlation.pdf}
    % \caption{The .}
    \label{figure:human_eval_scores}
 \end{subfigure}
\hfill
 \begin{subfigure}[b]{0.5\textwidth}
\centering
    \includegraphics[width=\textwidth]{figures/resources/human_eval_results_feedback.pdf}
    % \caption{The distribution of the score criteria analyzed with Topic Modeling.}
    \label{figure:human_eval_feedback}
 \end{subfigure}
 \caption{}
 \label{}
\end{figure*}

==> sections/unused-training-prometheus.tex <==
\section{Training Prometheus}
Prometheus, our model, stands at the core of this research. Herein, we elaborate on the fine-tuning process for the intricate task of text evaluation that we employed, which blends our extensive dataset and standard training methodologies.

% 2. Initial Setup

a. Model Selection: Our starting point involved choosing an appropriate language model for fine-tuning. For this study, we opted for Llama-2 as our base model, intending to refine its capabilities into a proficient LLM Judge.

% 3. Feedback Collection Instance Splitting

The feedback collection instances, each containing an instruction, a reference answer, a scoring rubric, and five candidate responses mapped with feedback and scores, demanded restructuring for training purposes.

a. Segregation Strategy: We divided each Feedback Collection instance into five distinct training instances. This division was grounded in the scores, meaning each training instance showcased:

A single instruction
One scoring rubric
A reference answer
One candidate response (from the original set of five) that the model is tasked with evaluating
Associated feedback
The corresponding score
Through this division, our intention was to offer the model a granular perspective, enabling it to focus on individual responses and their respective scores in isolation.

4. Training Mechanics

Once our training dataset was structured, the subsequent steps were straightforward.

a. Causal Language Model Training: While Prometheus's training utilizes causal language modeling principles, it's imperative to emphasize that we only propagated the loss to the components responsible for feedback and score generation. By doing so, we ensured that the model's primary focus was honed in on these crucial evaluation aspects.

b. Hyperparameters: To maintain simplicity and consistency in our approach, we refrained from intricate hyperparameter tuning. The specific values and configurations that we adhered to are documented in the appendix for transparency and replicability.

5. Conclusion

The training process of Prometheus, though seemingly straightforward, encapsulates deliberate choices and methodologies. The goal was to equip the model with a sharp focus on evaluation, feedback, and score generation, pivotal components in assessing text as dictated by our rubrics. While the basic training structure forms the foundation, the exploration into different components' importance is undertaken in subsequent sections, where we deep dive into specific experiment settings and probe our research questions.

==> tables/rouge.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\caption{Rouge-1 and -L scores.}
\begin{tabular}{@{}lll@{}}
\toprule
Metrics                 & Mean Score & Standard Deviation \\ \midrule
ROUGE-1 Train         & 0.2544     & 0.0999             \\
ROUGE-1 Test          & 0.2995     & 0.1408             \\
ROUGE-1 Mixed         & 0.2516     & 0.0951             \\ \midrule
ROUGE-L Train         & 0.2226     & 0.0895             \\
ROUGE-L Test          & 0.2417     & 0.1351             \\ 
ROUGE-L Mixed         & 0.2104     & 0.0787            \\ \bottomrule
\end{tabular}
\label{tab:rouge}
\end{table}
